Matryoshka Quantization

Quantizing model weights is critical for reducing the communication and inference costs of large models. However, quantizing models -- especially to low precisions like int4 or int2 -- requires a trade-off in model quality; int2, in particular, is known to severely degrade model quality. Consequently, practitioners are often forced to maintain multiple models with different quantization levels or serve a single model that best satisfies the quality-latency trade-off. On the other hand, integer data types, such as int8, inherently possess a nested (Matryoshka) structure where smaller bit-width integers, like int4 or int2, are nested within the most significant bits. Leveraging this insight, in this paper, we propose Matryoshka Quantization (MatQuant), a novel multi-scale quantization technique that alleviates the aforementioned challenge. This technique allows us to train and maintain a single quantized model but serve it with the precision demanded by the deployment. Furthermore, leveraging MatQuant's co-training and co-distillation regularization, int2 precision models extracted by MatQuant outperform standard int2 quantization by up to to 4% and 7% with OmniQuant and QAT as base algorithms respectively. Finally, we demonstrate that by using an extra bit to represent outliers, a model with an effective precision of 2.05-bit gives an additional 6% improvement with OmniQuant as the base algorithm.

==> TabsNFigs/FakeQuant_Gemma_9B/table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\caption{Table presents downstream evaluation and perplexity results for \spalg, comparing it with \alg and the  \textit{Baseline} for int2, int4 and int8 quatization of Gemma-2 9B with OmniQuant and QAT. Note that the model was trained for int2 with \spalg, and the int4 and int8 models were sliced post training using Equation~\ref{eqn:matquant}.}
\label{sp_9B}
\begin{tabular}{@{}ccccccccc@{}} \toprule
\multicolumn{1}{l}{}       & int2      & \multicolumn{7}{c}{Gemma2-9B}                                            \\ \midrule
\multicolumn{1}{l}{}       & Method     & ARC-c   & ARC-e   & BoolQ   & HellaSwag & PIQA    & Winogrande & Task Avg. \\ \midrule
\multirow{3}{*}{OmniQuant} & S.P. \alg & $49.74$ & $74.66$ & $80.92$ & $66.57$   & $76.06$ & $63.54$    & $68.58$ \\
                           & Baseline   & $39.16$ & $63.43$ & $72.11$ & $52.24$   & $72.63$ & $61.88$    & $60.24$ \\
                           & \alg  & $48.72$ & $72.18$ & $79.2$  & $68.11$   & $76.17$ & $66.77$    & $68.52$ \\ \midrule
\multirow{3}{*}{QAT}       & S.P. \alg & $41.21$ & $66.2$  & $65.02$ & $64.31$   & $76.06$ & $62.35$    & $62.53$ \\
                           & Baseline   & $33.45$ & $55.43$ & $62.26$ & $54.8$    & $70.51$ & $59.67$    & $56.02$ \\
                           & \alg  & $39.85$ & $65.66$ & $65.93$ & $64.08$   & $75.68$ & $62.75$    & $62.32$ \\ \bottomrule
\end{tabular}
\end{table*}

==> TabsNFigs/Older_OmniQuant_main_paper_evals/table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}
% \centering
% \vspace{-3mm}
\caption{Average number of bits for \alg (with OmniQuant as the base algorithm) when sliced with Equation~\ref{eqn:slicing_old} instead of Equation~\ref{eqn:slicing}.} 
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{@{}cccccccc@{}}
\toprule
Data type              & \multicolumn{1}{c}{Gemma-2 2B} & \multicolumn{1}{c}{Gemma-2 9B} & \multicolumn{1}{c}{Mistral 7B} \\\midrule
\multicolumn{1}{l}{}  & Avg. Bits   & Avg. Bits  & Avg. Bits    \\\midrule
\multirow{1}{*}{int6} 
                       & $6.018$        & $6.018$        & $6.018$        \\
\multirow{1}{*}{int4} 
                       & $4.023$        & $4.022$       & $4.022$        \\
\multirow{1}{*}{int3} 
                       & $3.031$         & $3.029$        & $3.030$        \\
\multirow{1}{*}{int2} 
                       & $2.052$       & $2.050$       & $2.051$       \\
 \bottomrule
\end{tabular}
\label{tab:avg_bits}
}
% \vspace{-4mm}
\end{table}

==> TabsNFigs/QATFFNATTN_Gemma9B_Mistral7B_Alldatasets/table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\caption{QAT FFN + ATTN FakeMat for 2bit 3bit Gemma-2 9B} 
\begin{tabular}{@{}ccccccccc@{}} \toprule
DataType             & Method               & \multicolumn{7}{c}{Gemma-2 9B}                                           \\ \midrule
\multicolumn{1}{l}{}   & \multicolumn{1}{l}{} & ARC-c   & ARC-e   & BoolQ   & HellaSwag & PIQA    & Winogrande & Task Avg. \\ \midrule
\multirow{3}{*}{int2} & Baseline                 & $24.91$ & $41.62$ & $62.26$ & $40.87$   & $63.38$ & $53.67$    & $47.78$ \\
                       & Sliced int8       & $24.74$ & $25.63$ & $58.53$ & $25.5$    & $50.71$ & $49.17$    & $39.05$ \\
                       & \alg            & $28.24$ & $39.23$ & $62.17$ & $39.13$   & $63.49$ & $50.75$    & $47.17$ \\ \midrule
\multirow{3}{*}{int3} & Baseline                 & $50.85$ & $73.11$ & $71.13$ & $72.01$   & $79.38$ & $65.67$    & $68.69$ \\
                       & Sliced int8       & $43.6$  & $64.98$ & $72.66$ & $66$      & $75.95$ & $62.19$    & $64.23$ \\
                       & \alg            & $45.22$ & $69.32$ & $78.5$  & $68.72$   & $76.01$ & $63.85$    & $66.94$ \\ \bottomrule
\end{tabular}
\end{table*}

==> TabsNFigs/QATFFNATTN_Gemma9B_Mistral7B_Alldatasets/table4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\caption{QAT FFN + ATTN FakeMat for 2bit 3bit Mistral 7B}
\begin{tabular}{@{}ccccccccc@{}} \toprule
Bit width              & Method               & \multicolumn{7}{c}{Mistral 7B}                                           \\ \toprule
\multicolumn{1}{l}{}   & \multicolumn{1}{l}{} & ARC-c   & ARC-e   & BoolQ   & HellaSwag & PIQA    & Winogrande & Average \\ \midrule
\multirow{3}{*}{int2} & Baseline                  & $23.21$ & $23.82$ & $37.83$ & $24.67$   & $49.02$ & $49.57$    & $34.69$ \\
                       & Sliced int8        & $22.78$ & $24.03$ & $58.75$ & $24.63$   & $50.54$ & $49.64$    & $38.39$ \\
                       & \alg            & $22.27$ & $32.49$ & $62.02$ & $32.43$   & $59.3$  & $51.46$    & $43.33$ \\ \midrule
\multirow{3}{*}{int3} & Baseline                  & $41.98$ & $65.53$ & $79.39$ & $74.42$   & $79.22$ & $69.93$    & $68.41$ \\
                       & Sliced int8        & $20.65$ & $31.57$ & $44.34$ & $28.79$   & $59.41$ & $51.38$    & $39.36$ \\
                       & \alg            & $34.64$ & $55.13$ & $70.43$ & $58.61$   & $73.39$ & $64.48$    & $59.45$ \\ \bottomrule
\end{tabular}
\end{table*}

==> TabsNFigs/QATFFNATTN_Gemma9B_Mistral7B_Average_logpplx/table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\caption{FFN + ATTN FakeMat for 2bit 3bit}
\begin{tabular}{@{}cccccc@{}} \midrule
Bit width              & Method               & \multicolumn{2}{c}{Gemma-2 9B} & \multicolumn{2}{c}{Mistral 7B} \\ \midrule
\multicolumn{1}{l}{}   & QAT & Average       & log pplx.      & Average       & log pplx.      \\ \midrule
\multirow{3}{*}{2-bit} & Baseline                 & $47.78$       & $3.7$          & $34.69$       & $7.56$         \\
                    %   & 8-bit + Slicing       & $39.05$       & $13.12$        & $38.39$       & $12.07$        \\
                       & MatQuant             & $47.17$       & $3.84$         & $43.33$       & $3.81$         \\ \midrule
\multirow{3}{*}{3-bit} & Baseline                 & $68.69$       & $2.57$         & $68.41$       & $2.24$         \\
                    %   & 8-bit + Slicing       & $64.23$       & $2.91$         & $39.36$       & $4.92$         \\
                       & MatQuant             & $66.94$       & $2.91$         & $59.45$       & $2.7$      \\ \midrule   
\end{tabular}
\end{table*}
